On the Capacity of SWIPT Systems with a Nonlinear Energy Harvesting Circuit

In this paper, we study information-theoretic limits for simultaneous wireless information and power transfer (SWIPT) systems employing a practical nonlinear radio frequency (RF) energy harvesting (EH) receiver. In particular, we consider a three-node system with one transmitter that broadcasts a common signal to separated information decoding (ID) and EH receivers. Owing to the nonlinearity of the EH receiver circuit, the efficiency of wireless power transfer depends significantly on the waveform of the transmitted signal. In this paper, we aim to answer the following fundamental question: What is the optimal input distribution of the transmit waveform that maximizes the rate of the ID receiver for a given required harvested power at the EH receiver? In particular, we study the capacity of a SWIPT system impaired by additive white Gaussian noise (AWGN) under average-power (AP) and peak-power (PP) constraints at the transmitter and an EH constraint at the EH receiver. Using Hermite polynomial bases, we prove that the optimal capacity-achieving input distribution that maximizes the rate-energy region is unique and discrete with a finite number of mass points. Furthermore, we show that the optimal input distribution for the same problem without PP constraint is discrete whenever the EH constraint is active and continuous zero-mean Gaussian, otherwise. Our numerical results show that the rate-energy region is enlarged for a larger PP constraint and that the rate loss of the considered SWIPT system compared to the AWGN channel without EH receiver is reduced by increasing the AP budget.

==> proof_outage_Nakagami.tex <==
\section{Proof of Proposition \ref{prop:outage_Nakagami}}
\label{App:proof_outage_Nakagami}
By using the pdf and the ccdf of the equivalent UL and DL channels from (\ref{eq:pdf}) and (\ref{eq:ccdf}) in (\ref{eq:Outage_general_finite_limits}) and defining $c_1=\lambda_1/(a\Pt)$ and $c_2=\lambda_2c(1+\e^{ab})$, we can write
$\bar{F}_{v_2}\!\!\left(\!\frac{c(1+\e^{ab}\!)}{y}\!-\!c\e^{ab}\!\right)=\e^{\lambda_2 c\e^{ab}}\!\e^{\frac{-c_2}{y}}\sum\limits_{k=0}^{m_2N_2-1}\!\!\frac{(\lambda_2c\e^{ab})^k}{k!}\!\!\sum\limits_{l=0}^k\!\!\binom{k}{l}(-1)^{k-l}(1\!+\!\e^{-ab})^l y^{-l}$ and
$f_{v_1}\!\!\left(\!\frac{-\ln(1\!-\!y)}{a\Pt}\!\right)=\frac{\lambda_1^{m_1N_1}}{\Gamma(m_1N_1)}\left(\frac{-\ln(1\!-\!y)}{a\Pt}\right)^{m_1N_1-1}(1-y)^{c_1}$, where we used the identities $\alpha\ln(z)=\ln(z^\alpha)$ and $\e^{\ln(z)}=z$. Thus, the outage probability in (\ref{eq:Outage_general_finite_limits}) reduces to\vspace{-0.2cm}
\begin{equation}
\begin{aligned}
&\pout\!\!=\!1\!-\!\!\frac{c_1(-1)^{m_1N_1\!-\!1}}{\Gamma(m_1N_1)}\e^{\lambda_2c\e^{ab}}\!\!\!\sum\limits_{k=0}^{m_2N_2-1}\!\!\frac{(\lambda_2c\e^{ab})^k}{k!}\!\sum\limits_{l=0}^{k}\!\!\binom{k}{l}\!(-\!1)^{k\!-\!l}\\[-1ex]
&(1\!+\!\e^{-ab})^l \!\!\int_{0}^{1}\!\!\left[c_1\ln(1-y)\right]^{\!m_1N_1\!-\!1}(1\!-\!y)^{c_1-1}\e^{\frac{-c_2}{y}}y^{-l} \dd y.\!\\[-2ex]
\end{aligned}
\label{eq:Pout_step}
\end{equation}
In order to solve the integral in (\ref{eq:Pout_step}), we use the relation $\frac{\partial^{n}}{\partial s^{n}}Z^{q s}=[q\ln(Z)]^n  Z^{q s}$ at $Z\!=\!1\!-\!y$, $n\!=\!m_1N_1\!-\!1$, and $q\!=c_1$ and use the following substitution $\left[c_1\ln(1\!-\!y)\right]^{\!m_1N_1\!-\!1}(1\!-\!y)^{c_1}=\frac{\partial^{m_1N_1\!-\!1} (1-y)^{c_1s}}{\partial s^{m_1N_1\!-\!1}}\!\Big|_{s=\!1}$. By swapping the order of integration and differentiation, the integral in (\ref{eq:Pout_step}) reduces to $\frac{\partial^{m_1N_1\!-\!1} }{\partial s^{m_1N_1\!-\!1}}I_s\big|_{s=\!1}$, where $I_s=\int_{0}^{1}(1\!-\!y)^{c_1s-1}\e^{\frac{-c_2}{y}}y^{-l} \dd y$. Using \cite[Eq. 3.471.2]{table_of_integrals_Ryzhik}, $I_s$ reduces to $I_s=c_2^{-\frac{l}{2}}\e^{-\frac{c_2}{2}}\Gamma(c_1 s)W_{\frac{l}{2}-c_1 s,\frac{l}{2}-\frac{1}{2}}(c_2)$, where we used $W_{\alpha,\beta}(z)=W_{\alpha,-\beta}(z)$ given in \cite[Eq. 9.232.1]{table_of_integrals_Ryzhik}. Using the relation between the Whittaker W function and the confluent hypergeometric function $W_{\alpha,\beta}(z)=z^{\beta+\frac{1}{2}}\e^{-\frac{z}{2}}U(\beta-\alpha+1/2,2\beta+1,z)$ \cite[Eq. 9.220.2]{table_of_integrals_Ryzhik}, $I_s$ reduces to $I_s=\e^{-c_2}\Gamma(c_1 s)U(c_1 s,l,c_2)$. Replacing the integral in (\ref{eq:Pout_step}) by $\frac{\partial^{m_1N_1\!-\!1} }{\partial s^{m_1N_1\!-\!1}}I_s\big|_{s=\!1}$ and using $c_1=\lambda_1/(a\Pt)$ and $c_2=\lambda_2c(1+\e^{ab})$, the outage probability reduces to  (\ref{eq:Outage_Nakagami}). Next, we prove the asymptotic outage probability in (\ref{eq:asym_Pout}). In the limit as $\Pt\to\infty$, the harvested power saturates at $\PEH\to M$. Hence, the outage probability simplifies to  $\pout=\pr(\frac{\theta M\tau v_2}{(1-\tau)\sigma^2}<\gammathr)=\pr(v_2<c)=1-\bar{F}_{v_2}(c)$, where $\bar{F}_{v_2}(c)$ is given in (\ref{eq:ccdf}). Finally, the asymptotic throughput follows directly from (\ref{eq:throughput}). This completes the proof.
